Analysis of Linear Difference Schemes in the Sparse Grid Combination Technique

Sparse grids are tailored to the approximation of smooth high-dimensional functions. On a $d$-dimensional tensor product space, the number of grid points is $N = \mathcal O(h^{-1} |\log h|^{d-1})$, where $h$ is a mesh parameter. The so-called combination technique, based on hierarchical decomposition and extrapolation, requires specific multivariate error expansions of the discretisation error on Cartesian grids to hold. We derive such error expansions for linear difference schemes through an error correction technique of semi-discretisations. We obtain overall error formulae of the type $\epsilon = \mathcal{O} (h^p |\log h|^{d-1})$ and analyse the convergence, with its dependence on dimension and smoothness, by examples of linear elliptic and parabolic problems, with numerical illustrations in up to eight dimensions.

==> DuenneGitter.tex <==
\ueberblick{
In den vorangegangenen Kapiteln wurden klassische Diskretisierungsmethoden für
parabolische Gleichungen und deren effiziente Mehrgitterlösung
diskutiert, wobei festzustellen war, dass in mehr als drei
Raumdimensionen der exponentiell steigende Aufwand für hinreichend
exakte Lösungen in vernünftiger Zeit undurchführbar wird.

In Abschnitt \ref{sec:sparsegrid} wird zunächst erläutert, wie der "`Fluch
der Dimension"' durch Approximation in sog.\ \emph{Dünngitterräumen} durchbrochen
werden kann, was mit jüngsten Anwendungen auf Optionspreisaufgaben
untermauert wird.

Für die Kombinationstechnik, einem darauf basierenden
Extrapolationsalgorithmus, werden in Abschnitt \ref{sec:combi}
Konvergenzabschätzungen in einer geschlossenen Form für allgemeine
Dimensionen bewiesen, was das mathematische Herzstück dieser Arbeit
darstellt.
%Anhand von
%parallelen numerischen Experimenten werden die 
%auf heutigen Rechnern behandelbaren Dimensionalitäten ausgelotet.

%Durch multivariate Extrapolation wird in \ref{sec:multiextra} aus einer
%Diskretisierung zweiter Ordnung ein Verfahren vierter Ordnung
%gewonnen, um es in \ref{sec:highord} zusammen mit den Resultaten aus
%\ref{sec:combi} zu einer entsprechenden Dünngittermethode zu verweben.
}

\section{Das Prinzip d\"unner Gitter}
\label{sec:sparsegrid}

Betrachtet man in $d$ Dimensionen ein kartesisches Gitter mit $n$
 Punkten in jede Richtung, so läßt sich etwa durch multilineare
 Ansatzfunktionen (für hinreichend glatte Funktionen) ein
 Approximationsfehler von $\epsilon =
 \mathcal{O}(n^{-2})$ für den Preis von $n^d$ Freiheitsgraden
 erreichen. Ansätze höherer Ordnung drücken den Aufwand (bei
 vorausgesetzter Glattheit), kommen aber um das prinzipielle Problem
 exponentiell ansteigenden Aufwands nicht herum.

 D\"unne Gitter eignen sich unter noch stärkeren Regularit\"atsvoraussetzungen
 zur Approximation in
 h\"oheren Raumdimensionen mit einer substantiell geringeren Anzahl an
 Freiheitsgraden.
 Dem Ansatz liegt eine Approximation \"uber
 hierarchische Tensorproduktbasen zugrunde.
 Sei dazu $V$ ein vollst\"andiger (separabler) Raum, der eine Darstellung als
 (abgeschlossene) direkte Summe von endlichdimensionalen Räumen der
 Gestalt
 %\[
 %V = \overline{\biguplus_{n=1}^\infty \bigoplus_{k_j \le n}
 %  \bigotimes_{j=1}^d U_{n_j}^j}
 %\]
 \[
 V^{(n_1,\ldots,n_d)} := V_{n_1}^{(1)} \times \cdots \times
 V_{n_d}^{(d)}
 \]
 mit $n_j \in \N_0$ hat.
 Ein volles Gitter entspricht dann einer Folge von Unterr\"aumen
 \[
 V^{(n)} := \bigoplus_{\scriptsize \begin{array}{c} n_k\le n
 %, \\ 1\le k\le d
 \end{array}} V^{(n_1,\ldots,n_d)},
 \]
 f\"ur das d\"unne Gitter w\"ahlt man hingegen
 \[
 \hat{V}^{(n)} := \bigoplus_{\scriptsize \begin{array}{c} \sum_k n_k\le n
 %, \\ 1\le k\le d 
 \end{array}} V^{(n_1,\ldots,n_d)}.
 \]


 %Sei dazu $V$ ein vollst\"andiger Raum und sei die Vereinigung der
 %\[
 %V^{(n_1,\ldots,n_d)} := V_{n_1}^{(1)} \times \cdots \times
 %V_{n_d}^{(d)}
 %\]
 %mit $n_i \in \N_0$ dicht in $V$. Ein volles Gitter enspricht dann
 %einer Folge von Unterr\"aumen
 %\[
 %V^{(n)} := \bigcup_{\scriptsize \begin{array}{c} n_k\le n
 %\end{array}} V^{(n_1,\ldots,n_d)},
 %\]
 %f\"ur das d\"unne Gitter w\"ahlt man hingegen
 %\[
 %\hat{V}^{(n)} := \bigcup_{\scriptsize \begin{array}{c} \sum_k n_k\le n
 %\end{array}} V^{(n_1,\ldots,n_d)}.
 %\]

 Betrachten wir als Spezialfall $V=H^1_0\big([0,1]^d\big)$ und
 \[
 V^{(i)}_{n_i}:= \Big\{v: [0,1]\rightarrow \R \Big| v \text{ ist st\"uckweise linear mit
   St\"utzstellen } \frac{j}{2^{n_i}}, 0\le j \le 2^{n_i} \Big\}.
 \]
Die Abbildungen \ref{full-fig} und \ref{sparse-fig} zeigen die
 entsprechenden Gitter für $d=2$.
% \begin{center}
 {\setlength{\unitlength}{1.5 cm}
 \begin{figure}
 \setcapindent{2 em}
 \begin{center}
 \input{Numerik/fullgrid.tex}
 \end{center}
 \caption{Zweidimensionale Vollgitterhierarchie, dargestellt sind die
   Freiheitsgrade der hierarchischen Basis als Knoten. Die
   Anzahl steigt in $d$ Dimensionen mit $2^{nd}$.}
 \label{full-fig}
 \end{figure}
 %\end{center}
 %\begin{center}
 \begin{figure}
 \setcapindent{2 em}
 \begin{center}
   \setlength{\unitlength}{1.5 cm}
   \input{Numerik/sparsegrid.tex}
 \caption{Zweidimensionale D\"unngitterhierarchie. Der Raum auf jeder
   Stufe $n\ge 0$ entspricht einer Familie von Gittern.
 Die Anzahl der Knoten pro Gitter steigt in $d$ Dimensionen nur mit
   $\mathcal{O}(2^n)$, die der Gitter mit $\mathcal{O}(n^{d-1})$.}
 \label{sparse-fig}
 \end{center}
 \end{figure}
 %\end{center}
 }

\clearpage

 Es ist einsichtig, dass es auf Stufe $n$
 \begin{equation}
 \label{nGrids}
 N = \bino{n+d-1}{d-1}
 \end{equation}
 Gitter
 mit jeweils genau $2^n$ Elementen und $\mathcal{O}(2^n)$ Knoten
 gibt. Die Anzahl der Unbekannten steigt also nur nach
 \begin{equation}
\label{log-lin-com}
 N_n^{(d)} = \mathcal{O}(n^{d-1} 2^n).
 \end{equation}

 Bungartz \cite{bungartz:92} zeigt f\"ur den entsprechenden
 multilinearen Interpolanden $u_n$ die Absch\"atzung
 \begin{equation}
 \label{bungee}
 \|u-u_n\|_\infty \le \frac{1}{6^d} \left\|\frac{\partial^{2d} u}
 {\partial x_1^2 \ldots \partial x_d^2}\right\|_\infty
 \left(1+\sum_{i=1}^{d-1} \left(\frac{3}{4}\right)^i
 \cdot \bino{n+i-1}{i}\right) h_n^2
 \end{equation}
 f\"ur Funktionen mit derart beschr\"ankten gemischten
 Ableitungen.
 Der D\"unngitterraum $\hat{V}^{(n)}$ hat damit die
 Approximationseigenschaft
 \[
 d_\infty(u,\hat{V}^{(n)}) = \mathcal{O}(h_n^2 (\ln_2 h_n^{-1})^{d-1})
 \]
 mit $h_n=2^{-n}$ f\"ur hinreichend glatte $u$ (d.~h.\ mit beschränkten
 gemischten zweiten Ableitungen). Die Verschlechterung zum vollen Raum
 $V^{(n)}$ besteht nur in logarithmischen Faktoren.

 Dieses Approximationsresultat und Varianten davon k\"onnen auf mehrere
 Weisen zur effizienten L\"osung von Aufgabenstellungen hoher
 (in der Praxis: moderater) Dimension angewandt werden.
 Über die reine Approximation (\emph{Data Mining}) hinaus sind die
 Resultate zur Integration und zur Lösung partieller
 Differentialgleichungen nützlich.
 Im Folgenden ein
 kurzer Streifzug mit speziellem Fokus auf Anwendungen aus der
 Finanzmathematik.


 \subsubsection{D\"unngitter-Integration}

 Dünne Gitter tauchen schon in den Sechziger-Jahren bei Smolyak
 \cite{smolyak:63} zur Integration von Funktionen in
 Tensorprodukträumen auf. Es ist offensichtlich, wie das
 Approximationsresultat (\ref{bungee}) auf entsprechende Produkte von Quadraturformeln
 zu übertragen ist.

 Anwendungen auf Probleme der Finanzmathematik wurden von Griebel und
 Gerstner \cite{gerstner-griebel} behandelt. Im Fall von Europäischen
 Optionen kann dazu die Integraldarstellung
 (\ref{green-representation}) des Black-Scholes-Preises
 mittels Greenscher Funktion herangezogen werden.

% dass der Preis
% einer Europ\"aischen Option als
% diskontierter Erwartungswert der
% Auszahlungsfunktion --- also als Integral nach einem risikoneutralen
% Wahrscheinlichkeitsmaß ---
% bzw. konkreter als Faltung der Anfangsbedingung mit der Greenschen
% Funktion der Wärmeleitungsgleichung 
% (unter Verwendung der Transformation (\ref{x-eqn})) dargestellt werden kann:

% Der Zusammenhang zur partiellen Differentialgleichung wird über den
% Feynman-Kac-Formalismus hergestellt.

In \cite{gerstner-griebel:03} verwenden sie dazu eine Heuristik für die Verteilung
 der Freiheitsgrade auf die Raumrichtungen ("`dimensionsadaptive"'
 d\"unne Gitter).

 \subsubsection{D\"unngitter-Finite Elemente}

 Bungartz zeigt Approximationsresultate wie (\ref{bungee}) f\"ur
 Elemente erster
 \cite{bungartz:92}
 und h\"oherer Ordnung \cite{bungartz:98} und \"ubertr\"agt diese
 Absch\"atzungen \"uber einen Standard-Galerkin-Ansatz vermöge
 klassischer Orthogonalitätsprinzipien auf
 Finite-Elemente-Konvergenzresultate der Gestalt
\begin{equation}
\label{bungi}
\|u-u_n\|_1 \le c(d) |\log h_n|^{d-1} h_n^p.
\end{equation}
Entscheidender Nachteil ist die
 fehlende Lokalität des diskreten Operators, was sich in der
 Besetztheitsstruktur der Steifigkeitsmatrix niederschlägt.

 Petersdorff und Schwab \cite{petersdorff-schwab:02} wählen einen
 ähnlichen Zugang mit Wavelet-Basen.
 Durch Approximation der Koeffizienten mit Polynomen und spezielle
 rekursive Auswertung können sie (wie auch \cite{bungartz:92} für
 die Laplace-Gleichung, aber in einem allgemeineren Kontext) trotzdem
 lineare Komplexität für die
 Matrix-Vektor-Multiplikation erreichen.  Außderdem erhalten sie selbst
 bei reduzierter Regularität der Anfangsbedingung ($u_0 \in H^\epsilon$
 mit $\epsilon > 0$, wie es für Optionspreisaufgaben typisch ist) durch
 die Glättungseigenschaft des Operators für Elemente der Ordnung $p$
  eine $L^2$-Fehlerasymptotik der Form $\mathcal{O}(h^{\theta_0 p +
    \delta})$, wobei $\delta = p/((p+1)d-1)$ ist und $\theta_0 \in (0,1]$
    mit der Regularität des Problems zusammenhängt.



\section{Die Kombinationstechnik}
\label{subsec:combi}

 In \cite{griebel-schneider-zenger} wird eine auf der D\"unngitterhierarchie
 basierende Extrapolationstechnik eingef\"uhrt, die dieselben
 asymptotischen Eigenschaften im Hinblick auf (\ref{log-lin-com}) und ---
 wie wir sehen werden --- auch (\ref{bungee}) aufweist, bei der aber nur
 Gleichungen auf kartesischen Gittern gelöst werden müssen.
 Der Vorzug der Methode vom praktischen Standpunkt besteht darin, dass
 die einzelnen Probleme v\"ollig
 entkoppelt parallel mit einer Methode der Wahl gerechnet werden
 können.
 F\"ur die Konvergenz der
 D\"unngitterl\"osung ist dabei die Fehlerasymptotik der Skelettl\"osungen auf den
 einzelnen Gittern, die in Abbildung \ref{sparse-fig} für $d=2$
 dargestellt sind, entscheidend.

\subsubsection{Der zweidimensionale Fall}

Zur Motivation dient der zweidimensionale Fall, da hier übersichtlich das
Prinzip deutlich wird.
Es ist naheliegend, bei Konvergenz zweiter Ordnung von einer
Fehlerasymptotik der Gestalt
\begin{eqnarray*}
u_{h_1,h_2} = u + \gamma_1(h_1) h_1^2 + \gamma_2(h_2) h_2^2 +
\gamma_{12}(h_1,h_2) h_1^2 h_2^2
\end{eqnarray*}
mit den zwei unabhängigen Gitterweiten $h_1$ und $h_2$ auszugehen.
Eine solche Abschätzung muss von der verwendeten Diskretisierung am
kartesischen Gitter kommen und wird z.~B.\ von Griebel et al.~für eine
Finite-Differenzen-Diskretisierung der zweidimensionalen
Laplace-Gleichung über Fourierreihen gezeigt
\cite{bungartz-griebel-roeschke-zenger:94}.

Betrachtet man die Gitterlösungen in Abb.\
\ref{sparse-fig} spaltenweise ($l=0,\ldots,n$ in Spalte $n$),
\begin{eqnarray*}
u_{2^{-l},2^{-n+l}} = u + \gamma_1(2^{-l}) 2^{-2l} + \gamma_2(2^{-n+l}) 2^{-2(n-l)} +
\gamma_{12}(2^{-l},2^{-n+l}) 2^{-2n},
\end{eqnarray*}
so fällt auf, dass der gemischte Term nur mehr das --- auf all diesen
Gittern gleiche --- Produkt der Gitterweiten $h_1 h_2 = 2^{-n}$ enthält.
Die Terme niedrigerer Ordnung können durch Summation
\begin{eqnarray*}
S_n &:=& \sum_{l=0}^n
u_{2^{-l},2^{-n+l}} \\
&=& (n+1) u + \sum_{l=0}^n \gamma_1(2^{-l}) 2^{-2l} +
\sum_{l=0}^n \gamma_2(2^{-l}) 2^{-2l} +
2^{-2n} \sum_{l=0}^n \gamma_{12}(2^{-l},2^{-n+l})
\end{eqnarray*}
und einen anschließenden Extrapolationsschritt
\begin{eqnarray}
\label{combi-2d}
u_n &:=& S_{n+1} - S_{n} \\
&=& u + \gamma_1(2^{-n-1}) 2^{-2n-2} + \gamma_2(2^{-n-1})
2^{-2n-2} \nonumber \\
&& \quad +
2^{-2n-2} \sum_{l=0}^{n+1} \gamma_{12}(2^{-l},2^{-n-1+l}) - 
2^{-2n} \sum_{l=0}^{n} \gamma_{12}(2^{-l},2^{-n+l})
\nonumber
\end{eqnarray}
zum Verschwinden gebracht werden.

Sind $\gamma_1$, $\gamma_2$, $\gamma_{12}$ sinnvollerweise
betragsmäßig beschränkt, etwa durch $K$, gilt also
\begin{eqnarray}
\nonumber
|u-u_n| &\le& K 4^{-n-1} + K 4^{-n-1} + K (n+2) 4^{-n-1} + K (n+1)
 4^{-n} \\
&=& K 4^{-n} \left(2 + \frac{5}{4} n \right).
\label{2dsg}
\end{eqnarray}
%\fixme{Vergleich mit Griebel!}


\subsubsection{Der allgemeine Fall}

In einer allgemeinen Dimension $d$
betrachten wir diskrete L\"osungen auf einer Hierarchie von
(anisotropen) kartesischen Gittern, charakterisiert
durch die (zunächst äquidistanten) Gitterweiten $\vf{h} =
(h_1,\ldots,h_d)$ in den einzelnen Raumrichtungen. Die dazugeh\"orige
Gitterl\"osung $u_{\vf{h}}$ wird wechselweise auch als $u_{\vf{i}}$
mit Multiindex $\vf{i}$ bezeichnet, wobei
dann $h_k = 2^{-i_k}$ gemeint ist.
Der Betrag f\"ur einen solchen Multiindex sei $|\vf{i}|: = \sum_{k=1}^d i_k$.

 
Die Kombinationstechnik fu{\ss}t dort ähnlich dem zweidimensionalen
Fall auf der Annahme einer
Fehlerasymptotik der Form
\begin{equation}
\label{asympt}
\fbox{$\displaystyle
u-u_{\vf h} = \sum_{m=1}^{d} 
\sum_{
\tiny \begin{array}{c}
\{j_1,\ldots,j_m\} \\
\subset \{1,\ldots,d\}
\end{array}}
\gamma_{j_1,\ldots,j_m}
(h_{j_1},\ldots, h_{j_m}) h_{j_1}^2\cdot \ldots \cdot h_{j_m}^2,
$}
\end{equation}
wobei die $\gamma_{j_1,\ldots,j_m}$ beschr\"ankt sein sollen,
d.~h.\ $|\gamma_{j_1,\ldots,j_m}|\le K$.

Eine natürliche Erweiterung der Kombinationsformel (\ref{combi-2d})
ist die iterierte Bildung von Differenzen benachbarter Spalten des
Gittertableaus.
F\"ur eine Funktion nat\"urlicher Zahlen $f: \N_0 \rightarrow \R$ sei also
 \[
 \Delta_n f: n \rightarrow f(n+1)-f(n) \quad \forall n \in \N_0.
 \]
Dann definiert sich die Kombinationsl\"osung auf Stufe $n$ als 
 \begin{equation}
 \label{combi-diff}
\fbox{$\displaystyle
 u_n := \Delta_n^{d-1} \sum_{|\vf{i}|=n} u_{\vf{i}}.
$}
 \end{equation}
 Iterierte Anwendung ergibt nach der binomischen Formel ($m\ge 0$)
 \[
 \Delta_n^m f(n) = \sum_{j=0}^m (-1)^{(m-j)} \bino{m}{j} f(n+j) \quad \forall n \in \N_0
 \]
und somit l\"a{\ss}t sich (\ref{combi-diff}) schreiben als
 \begin{equation}
 \label{combi}
 u_n = \sum_{l=n}^{n+d-1}  a_{l-n} \sum_{|\vf{i}|=l} u_{\vf{i}}
 \end{equation}
 mit
 \begin{equation}
 \label{combi-coeff}
 a_i := (-1)^{d-1-i} \bino{d-1}{i} \quad 0 \le i \le d-1.
 \end{equation}



 Griebel et al.\ zeigen in \cite{griebel-schneider-zenger}
 unter Verwendung von (\ref{combi}), (\ref{combi-coeff}) und unter der
 Voraussetzung (\ref{asympt}) punktweise Fehlerabsch\"atzungen 
 f\"ur den zweidimensionalen Fall,
 \begin{equation}
 \label{griebel-2d}
 |u-u_n| \le K h_n^2 \left(1 + \frac{5}{4} \log_2 h_n^{-1} \right),
 \end{equation}
(vergleiche (\ref{2dsg}) mit einer unterschiedlichen Indizierung der
 Gitter) und den dreidimensionalen Fall,
 \begin{equation}
 \label{griebel-3d}
 |u-u_n| \le K h_n^2 \left(1 + \frac{65}{32} \ld h_n^{-1} 
 + \frac{25}{32} (\log_2 h_n^{-1})^2 \right).
 \end{equation}
 Der dortige Zugang ist zwar prinzipiell \"ubertragbar auf
 beliebige (feste) h\"ohere Dimensionen, was angesichts der
 exponentiell ansteigenden Anzahl an Fehlertermen, die getrennt
 abgeschätzt werden müssen, allerdings schon in drei Dimensionen ein
 mühsames Unterfangen ist.

 Daher ist es erfreulich, dass im folgenden Abschnitt eine allgemeine
 Abschätzung in geschlossener Form für beliebige Dimensionen angegeben
 werden kann.




 \section{Konvergenzabschätzungen}
 \label{sec:combi}
 
In diesem Abschnitt wird der folgende zentrale Satz, ein
Pendant zu (\ref{griebel-2d}) und (\ref{griebel-3d})
in allgemeinen Dimensionen, hergeleitet.


\begin{satz}[Konvergenz zweiter Ordnung]
\label{zweiteOrdnung}
F\"ur alle L\"osungen $u_{\vf{h}}$ gelte punktweise eine Fehlerasymptotik der Form
\begin{equation}
\label{satz-asympt}
u-u_{\vf h} = \sum_{m=1}^d 
\sum_{\scriptsize \begin{array}{c}\{j_1,\ldots, j_m\} \\
\subset \{1,\ldots,d\} \end{array}}
\gamma_{j_1,\ldots,j_m}
(h_{j_1},\ldots, h_{j_m}) h_{j_1}^2\cdot \ldots \cdot h_{j_m}^2,
\end{equation}
wobei
\[
|\gamma_{j_1,\ldots,j_m}| \le K \quad \forall 1\le m\le d \; \forall
\{j_1,\ldots,j_m\} \subset \{1,\ldots,d\}.
\]
Dann erf\"ullt die Kombinationsl\"osung
\begin{equation}
%\label{satz-combi-diff}
u_n = \Delta_n^{d-1} \sum_{|\vf{i}|=n} u_{\vf{i}}
\end{equation}
die Fehlerabsch\"atzung
\begin{equation}
\fbox{$\displaystyle
\label{abschZweite}
|u-u_n| \le \frac{2 K}{(d-1)!} \left(\frac{5}{2}\right)^{d-1}
 (n+2(d-1))^{d-1} 4^{-n}.
$}
\end{equation}
\end{satz}


Vor dem eigentlichen Beweis werden noch vorbereitende Resultate gebracht.
Die folgende elementare Formel für
 Differenzen von Produkten --- eine diskrete Form der Leibniz-Regel
 --- wird dabei gelegentlich hilfreich sein.
 \begin{lemma}
 \label{prod-diff}
 Seien $f, g: \N_0 \rightarrow \R$, $f_n := f(n)$, $g_n:=g(n)$. Dann gilt
 \begin{equation}
 \Delta_n^k \left(f_n g_n\right) = \sum_{j=0}^k \bino{k}{j}
 \Delta_n^{k-j} f_{n+j} \Delta_n^j g_n \quad \forall k\in \N_0.
 \end{equation}
 \end{lemma}
 \begin{proof}
 Induktion nach $k$. $k=0$ ist klar, für $k=1$ gilt
 \begin{equation}
 \label{delta1d}
 \Delta_n \left(f_n g_n\right) = f_{n+1} g_{n+1} - f_n g_n = 
 f_{n+1} (g_{n+1} - g_n) + (f_{n+1} - f_n) g_n
 %f_{n+1} g_{n+1} - f_{n+1} g_n + f_{n+1} g_n - f_n g_n
 = f_{n+1} \Delta_n g_n +
 \Delta_n f_n g_n.
 \end{equation}
 Induktionsschritt $k \rightarrow k+1$:
 \begin{eqnarray*}
 \Delta_n^{k+1} \left(f_n g_n \right) &=& \Delta_n \Delta_n^{k}
 \left(f_n g_n\right) \\
 &=& \sum_{j=0}^k \bino{k}{j} \Delta_n \left[
 \Delta_n^{k-j} f_{n+j} \Delta_n^j g_n \right] \\
 &\stackrel{(\ref{delta1d})}{=}& \sum_{j=0}^k \bino{k}{j} \left[\Delta_n^{k-j} f_{n+j+1} \Delta_n^{j+1}
   g_n + \Delta_n^{k-j+1} f_{n+j} \Delta_n^j g_n \right] \\
 &=& \sum_{j=0}^k \bino{k}{j} \Delta_n^{k-j} f_{n+j+1} \Delta_n^{j+1}
   g_n + \sum_{j=0}^k \bino{k}{j} \Delta_n^{k-j+1} f_{n+j} \Delta_n^j g_n \\
 &=& \sum_{j=1}^{k+1} \bino{k}{j-1} \Delta_n^{k-j+1} f_{n+j}
   \Delta_n^j
   g_n + \sum_{j=0}^k \bino{k}{j} \Delta_n^{k-j+1} f_{n+j} \Delta_n^j
   g_n \\
 &=& \sum_{j=1}^k \left[\bino{k}{j-1} + \bino{k}{j} \right]
   \Delta_n^{k-j+1} f_{n+j} \Delta_n^j + 
 \bino{k}{0} \Delta_n^{k+1} f_n \Delta_n^0 g_n \\
 && + \bino{k}{k} \Delta_n^0 f_{n+k+1} \Delta_n^{k+1} g_n \\
 &=& \sum_{j=0}^{k+1} \bino{k+1}{j}
 \Delta_n^{k+1-j} f_{n+j} \Delta_n^j g_n
 \end{eqnarray*}
 \end{proof}

 Da die Zahl der Gitter auf Stufe $n$ in $d$ Dimensionen durch (\ref{nGrids})
 gegeben ist, liefert das folgende Lemma \ref{konsistenz} (mit der
 Umbenennung $n+d-1 \rightarrow n$) eine
 notwendige Bedingung f\"ur die Konsistenz der Kombinationsformel (d.~h.\
 die Summe der Koeffizienten ist $1$):
 %($n+d-1 \rightarrow n$):
 \begin{lemma}[Konsistenz]
 \label{konsistenz}
 $\forall d\in \N$, $\forall n\in \N, n>d-1$  gilt:
 \[
% \sum_{j=0}^{d-1} (-1)^{d-1-j} \bino{d-1}{j} \bino{n+j}{d-1} =
\Delta_n^{d-1} \bino{n}{d-1} = 1
 \]
 \end{lemma}
 \begin{proof}
 %Der erste Teil entspricht genau der binomischen Formel.
 F\"ur alle $n> d-1$, $0 \le k \le d-1$ gilt
 \[
 \Delta_n^k \bino{n}{d-1} = \bino{n}{d-k-1},
 \]
 wie man induktiv ($k\rightarrow k+1$) aus
 \[
 \Delta_n^{k+1} \bino{n}{d-1} = \Delta_n \bino{n}{d-k-1} = \bino{n+1}{d-k-1} - \bino{n}{d-k-1} 
 = \bino{n}{d-k-2}
 \]
 sieht.
 Insbesondere ergibt sich
 \[
 \Delta_n^{d-1} \bino{n}{d-1} = \bino{n}{0} = 1.
 \]
 \end{proof}

 F\"ur den Konvergenzbeweis ist noch ein technisches Hilfsresultat
 vonn\"oten, das zunächst etwas unmotiviert scheint, aber im
 Satz \ref{zweiteOrdnung} an einer zentralen Stelle eingehen wird.

Grob gesprochen wird dort $F_n$ die Fehlerentwicklung auf einer
Spalte im Gittertableau sein, wobei $\delta_n$ dem Fehler einer
bestimmten Ordnung ($\delta_l \sim s_l 2^{-l}$) und der binomische
Faktor der Anzahl solcher Fehlerterme entspricht.
Entscheidend ist der zweite Teil des Lemma, demnach in der
Kombinationslösung nur mehr der Term höchster Ordnung übrigbleibt.

 %Die wesentliche Aussage ist in Teil \ref{alltech2}, dass durch
 %Differenzierung gewichteter
 %Reihen einer speziellen Gestalt nur das höchste Folgenglied
 %stehenbleibt.

 \begin{lemma}[Darstellungsformel]
\label{tech}
Seien $\delta_l \in \R \; \forall l \in \N_0$ beliebig,
\[
F_n := \sum_{l=0}^n \delta_l \bino{n-l+d-1}{d-1}.
\]
\begin{enumerate}
\item
\label{alltech1}
F\"ur $0\le k< d$ gilt
\[
\Delta_n^k F_n = G_n^k + H_n^k,
\]
wobei
\begin{eqnarray*}
G_n^k &:=& \left\{
\begin{array}{ll}
0 & k = 0 \\
\sum_{j=1}^k \delta_{n+j} \bino{d-j-1}{k-j} & k\ge 1 
\end{array}
\right. \\
H_n^k &:=&
\sum_{l=0}^n \delta_{l} \bino{n-l+d-1}{d-k-1}
\end{eqnarray*}
\item
\label{alltech2}
\[
\Delta_n^{d} F_n = \delta_{n+d}
\]
%\item
%\label{alltech3}
%F\"ur $k>d$
%\[
%\Delta_n^k F_n =
%\left(\frac{1}{4}-\frac{3}{4}\Delta_n\right)^{k-d}
%\gamma_{n+d}
%\]
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}
\item
Induktion nach $k$:
Klarerweise ($k=0$)
\[
\Delta_n^0 F_n = F_n = H_n^0 = G_n^0 + H_n^0.
\]
Da $F_n$ von der Gestalt $\sum_{l=0}^n f(l,n)$ ist, gilt
\[
\Delta_n F_n = f(n+1,n+1) -
\sum_{l=0}^n \left(f(l,n+1)-f(l,n)\right),
\]
also
\begin{eqnarray*}
\Delta_n F_n &=& \delta_{n+1} + \sum_{l=0}^n
\delta_l \left[\bino{n-l+d}{d-1}-\bino{n-l+d-1}{d-1} \right] \\
&=& \delta_{n+1} + \sum_{l=0}^n \delta_l \bino{n-l+d-1}{d} \\
&=& G_n^1 + H_n^1,
\end{eqnarray*}
der Fall $k=1$.

F\"ur $k>1$ ergibt sich im Induktionsschritt
\begin{eqnarray*}
\Delta_n G_n^k &=& \sum_{j=1}^k 
\left(\delta_{n+j+1}-\delta_{n+j} \right)
\bino{d-j-1}{k-j} \\
&=& \delta_{n+k+1} - \delta_{n+1} \bino{d-2}{k-1}
+ \sum_{j=2}^k \delta_{n+j} \left[
\bino{d-j}{k-j+1}-\bino{d-j-1}{k-j} \right] \\
&=& \sum_{j=2}^{k+1}\delta_{n+j}
\bino{d-j-1}{k-j+1} - \delta_{n+1}\bino{d-2}{k-1} \\
&=& G_n^{k+1} - \delta_{n+1}\bino{d-2}{k} 
- \delta_{n+1} \bino{d-2}{k-1} \\
&=& G_n^{k+1} - \delta_{n+1} \bino{d-1}{k}.
\end{eqnarray*}
Für $H_n^k$ gilt wiederum
\begin{eqnarray*}
\Delta_n H_n^k &=& \delta_{n+1} \bino{d-1}{d-k-1} + \sum_{l=0}^n
\delta_l \left[\bino{n-l+d}{d-k-1}-\bino{n-l+d-1}{d-k-1}\right]
\\
&=& \delta_{n+1} \bino{d-1}{k} + \sum_{l=0}^n
\delta_l \bino{n-l+d-1}{d-k-2} \\
&=& H_n^{k+1} + \delta_{n+1} \bino{d-1}{k}.
\end{eqnarray*}
Damit ($k\rightarrow k+1$) fügt sich alles zusammen als
\[
\Delta_n^{k+1} F_n = \Delta_n \Delta_n^k F_n = \Delta_n \left(G_n^k + H_n^k\right) =
\Delta_n G_n^k + \Delta_n H_n^k = G_n^{k+1} + H_n^{k+1}.
\]
\item
Nach \ref{alltech1}. ergibt sich für $k=d-1$
\[
\Delta_n^{d-1} F_n = \sum_{j=1}^{d-1} \delta_{n+j} + \sum_{l=0}^n \delta_l
\]
und damit
\[
\Delta_n^d F_n = \sum_{j=1}^{d-1} (\delta_{n+j+1}-\delta_{n+j}) +
\delta_{n+1} = \delta_{n+d}.
\]
\end{enumerate}
\end{proof}





\begin{proof}[Beweis für Satz \ref{zweiteOrdnung}]
Wegen Lemma \ref{konsistenz} kann man schreiben
\[
u-u_n = \Delta_n^{d-1} \sum_{|\vf{i}|=n} (u-u_{\vf{i}}).
\]
Dabei ist
\[
u-u_{\vf i} = \sum_{m=1}^{d} \sum_{\scriptsize \begin{array}{c}\{j_1,\ldots, j_m\} \\
\subset \{1,\ldots,d\} \end{array}} \gamma_{j_1,\ldots,j_m}
(2^{-i_{j_1}},\ldots, 2^{-i_{j_m}}) 4^{-i_{j_1}}\cdot \ldots \cdot 4^{-i_{j_m}}.
\]
Wir betrachten nun getrennt die einzelnen Fehlerterme aus
(\ref{satz-asympt}), o.~B.~d.~A.\ sei f\"ur einen beliebigen Term mit $m$ Faktoren
$j_k = k$ für $1\le k \le m$:
\begin{eqnarray*}
\sum_{|\vf{i}|=n} \gamma_{1,\ldots,m}(h_{i_1},\ldots,h_{i_m})
h_{i_1}^2 \ldots h_{i_m}^2
&=& 
\sum_{|\vf{i}|=n} \gamma_{1,\ldots,m}(2^{-i_1},\ldots,2^{-i_m})
4^{-\sum_{k=1}^m i_k} \\
&=& \sum_{l=0}^n 
\underbrace{
\sum_{\sum_{k=1}^m i_k = l}
\gamma_{1,\ldots,m}(2^{-i_1},\ldots,2^{-i_m})}_{=:s_l}
4^{-l}
\sum_{\sum_{k=m+1}^d i_k = n-l} 1 \\
&=& \sum_{l=0}^n s_l 4^{-l} \bino{n-l+d-m-1}{d-m-1},
\end{eqnarray*}
wobei $s_l$ eigentlich noch von $m$, ja sogar von der Gestalt des
Fehlerterms $\gamma_{1,\ldots,m}$ abhängt, was wir im Hinterkopf
behalten.
Aus Lemma \ref{tech}, \ref{alltech2}.\ ($d\rightarrow d-m$,
$\delta_l\rightarrow s_l 4^{-l}$)  folgt die zentrale
Identität
\begin{equation}
\label{dieFormel}
\Delta_n^{d-m} \sum_{|\vf{i}|=n}
\gamma_{1,\ldots,m}(h_{i_1},\ldots,h_{i_m})
h_{i_1}^2 \ldots h_{i_m}^2 = s_{n+d-m} 4^{-(n+d-m)}.
\end{equation}
Au{\ss}erdem gilt f\"ur alle $j\ge 0$
\[
\Delta_n^j 4^{-n} = \left(-\frac{3}{4}\right)^j 4^{-n},
\]
wie man sofort induktiv ($j\rightarrow j+1$) aus
\[
\Delta_n^{j+1} 4^{-n} = \left(-\frac{3}{4}\right)^j
\left(4^{-(n+1)}-4^{-n}\right) = \left(-\frac{3}{4}\right)^{j+1} 4^{-n}
\]
sieht. Damit folgt aus Lemma \ref{prod-diff}
\begin{eqnarray*}
\Delta_n^{m-1} \left[s_{n+d-m} 4^{-(n+d-m)}\right] &=& 
\sum_{j=0}^{m-1} \bino{m-1}{j} \Delta_n^j s_{n+d-m} \Delta_n^{m-1-j} 4^{-(n+d-m+j)}\\
&=& \sum_{j=0}^{m-1} \bino{m-1}{j} \Delta_n^j s_{n+d-m}
\left(\frac{-3}{4}\right)^{m-1-j} 4^{-(n+d-m+j)}\\
&=& 4^{-(n+d-1)} \sum_{j=0}^{m-1} \bino{m-1}{j} \left(-3\right)^{m-1-j}
\Delta_n^j s_{n+d-m} \\
&=& 4^{-(n+d-1)} \left(\Delta_n-3\right)^{m-1} s_{n+d-m} \\
&=& 4^{-(n+d-1)} \sum_{i=0}^{m-1} s_{n+d-m+i} \bino{m-1}{i}
(-4)^{m-1-i} \\
&=& 4^{-(n+d-1)} \sum_{i=0}^{m-1} s_{n+d-i-1} \bino{m-1}{i}
(-4)^{i}.
\end{eqnarray*}
Es sei bemerkt, dass bis zu diesem Punkt keine Abschätzungen getroffen wurden
und daher
\[
\Delta_n^{d-1}
\sum_{|\vf{i}|=n} \gamma_{1,\ldots,m}(h_{i_1},\ldots,h_{i_m})
h_{i_1}^2 \ldots h_{i_m}^2 =
4^{-(n+d-1)} \sum_{i=0}^{m-1} s_{n+d-i-1} \bino{m-1}{i}
(-4)^{i}
\]
mit
\[
s_l = \sum_{\sum_{k=1}^m i_k = l}
\gamma_{1,\ldots,m}(2^{-i_1},\ldots,2^{-i_m})
\]
eine exakte Darstellung der $m$-faktorigen Fehlerterme in der
Kombinationslösung ist. Der Clou dabei ist, dass die Faktoren $h_i$
hier nicht mehr getrennt auftreten, sondern nur mehr in der maximalen
Ordnung $h_1 \cdot \ldots \cdot h_n = 4^{-n}$, was die (zweite)
Ordnung der Kombinationslösung sicherstellt. Entscheidend war dabei
der Einsatz von Lemma \ref{tech} in (\ref{dieFormel}), wonach sich
die gemischten Fehlerterme niedriger Ordnung auf wundersame Weise
wegheben.

In der Folge müssen noch die Fehlerkoeffizienten abgeschätzt werden,
deren Summation auf die polynomialen Terme in $n$ führt.
Da aus $|\gamma_{1,\ldots,m}|\le K$
\[
|s_l| \le K \bino{l+m-1}{m-1} \Rightarrow \max_{i=0}^{m-1}|s_{n+d-i-1}|
 \le K \bino{n+d+m-2}{m-1}
\]
folgt und damit
\begin{eqnarray}
\label{absEst}
|\left(\Delta_n-3\right)^{m-1} s_{n+d-m}| &\le& \max_{i=0}^{m-1} |s_{n+d-i-1}|
\sum_{i=0}^{m-1} \bino{m-1}{i} 4^{i} \\
&\le& K \bino{n+d+m-2}{m-1} 5^{m-1},
\nonumber
\end{eqnarray}
gilt insgesamt
\begin{eqnarray}
\nonumber
\bigg|\Delta_n^{d-1} \sum_{|\vf{i}|=n}
\gamma_{1,\ldots,m}(h_{i_1},\ldots,h_{i_m})
h_{i_1}^2 \ldots h_{i_m}^2 \bigg|
&=&
4^{-(n+d-1)} \left|\left(\Delta_n-3\right)^m s_{n+d-m}\right| \\
\label{ersteUngl}
&\hspace{-4 cm} \le&\hspace{-2 cm}
4^{-(n+d-1)} 5^{m-1} K \bino{n+d+m-2}{m-1} \\
\label{zweiteUngl}
&\hspace{-4 cm} \le&\hspace{-2 cm}
4^{-(n+d-1)} 5^{d-1} K \bino{n+2(d-1)}{d-1} \\
\label{dritteUngl}
%\nonumber
&\hspace{-4 cm} <&\hspace{-2 cm}
4^{-n} \left(\frac{5}{4}\right)^{d-1} \frac{K}{(d-1)!} (n+2(d-1))^{d-1}.
\end{eqnarray}
Da $2^d-1$ Fehlerterme auftreten, ergibt sich zusammen
\[
|u-u_n| < \left(\frac{5}{2}\right)^{d-1} \frac{2 K}{(d-1)!} (n+2(d-1))^{d-1} 4^{-n}.
\]
\end{proof}

Betrachten wir zunächst die Aussage des Satzes \ref{zweiteOrdnung} 
für kleine Dimensionen.  Für
$d=1$, wo das dünne Gitter gleich dem vollen Gitter ist,
reduziert sich die Abschätzung auf $|u-u_n| \le 2 K 4^{-n}$
(die Ersetzung von $2^d-1$ durch $2^d$ am Ende erklärt den unnötigen
Faktor 2).
Im Fall $d=2$ ist der führende Fehlerterm durch (\ref{dritteUngl})
gegeben, sodass wir in der höchsten Potenz von $n$
\[
|u-u_n| \sim K \frac{5}{4} n 4^{-n}
\]
erhalten, was sich mit dem Resultat (\ref{griebel-2d}) deckt.
Analog ergibt sich in $d=3$ Dimensionen
\[
|u-u_n| \sim K \frac{1}{2} \left(\frac{5}{4}\right)^2  4^{-n} =
K \frac{25}{32}  n^2 4^{-n}
\]
in Übereinstimmung mit (\ref{griebel-3d}). Die Terme niedrigerer
Ordnung differieren durch Unterschiede bei der Indizierung der Gitter.
Ab (\ref{zweiteUngl}) wurden diese Terme überdies zur Vereinfachung
des Resultats nicht gesondert abgeschätzt.

Interessanter ist natürlich, wie sich (\ref{abschZweite}) für große
$d$ verhält.
Hält man $n$ fest, so kann man die Fakultät nach der Stirling-Formel
\[
k! \approx \sqrt{2 \pi k} \left(\frac{k}{e}\right)^k
\]
(siehe etwa \cite{bronstein-semendjajew:91} oder
\cite{heuser:91} für einen Beweis)
abschätzen und sieht, dass die dimensionsabhängigen Terme asymptotisch
mit $(5 \e)^d/\sqrt{d}$ gegen Unendlich streben.



\section{Verbesserte Konvergenzabschätzungen}



Es drängt sich die Frage auf, ob man die
Dimensionsabhängigkeit der Konstanten in (\ref{abschZweite}), Satz \ref{zweiteOrdnung}, durch
sorgfältigeres
Abschätzen weiter drücken kann. Ausgangspunkt müssen die
Ungleichungen (\ref{ersteUngl}) bis (\ref{dritteUngl}) sein.
Da die $s_l$ --- indem sie von den unbekannten Fehlerkoeffizienten
abhängen --- allgemein sind, werden sie dazu aus den Differenzen
separiert.


\begin{korollar}[zu Satz \ref{zweiteOrdnung}]
\label{supiAbsch}
\begin{enumerate}
\item
Unter den Voraussetzungen von Satz \ref{zweiteOrdnung} gilt für $d\ge
2$ auch die etwas schärfere Fehlerabschätzung
\[
|u-u_n| \le 2 K \left(\frac{5}{2}\right)^{d-1} \left(1+
(n+d-1) \frac{1+\ln(d-1)}{d-1}\right)^{d-1} 4^{-n}.
\]
\item
Darüberhinaus gilt die Abschätzung
\begin{equation}
\label{asymptImpro}
|u-u_n| \le \frac{K}{(d-1)!} \left(\frac{5}{4}\right)^{d-1} n^{d-1}
 4^{-n} \qquad \forall n\ge N
\end{equation}
für hinreichend großes N.
\item
%Sind zusätzlich
%die Fehlerterme $\gamma_{i_1,\ldots,i_m}$, $1\le m\le d$, $\{i_k\}
%\subset \{1,\ldots,d\}$ stetig in $\vf 0 \in \R^m$, so kann sogar
%die asymptotische Näherung
Ist zusätzlich
der Fehlerterm $\gamma_{1,\ldots,d}$ stetig in $\vf 0 \in \R^d$ mit
$\gamma_0 := \gamma_{1,\ldots,d}(0,\ldots,0) \ne 0$, so
kann sogar
die asymptotische Näherung
\begin{equation}
\label{traum}
|u-u_n| \sim \gamma_0 \left(\frac{3}{4}\right)^{d-1}
 \frac{n^{d-1}}{(d-1)!} 4^{-n}
\qquad \text{für } n \rightarrow \infty
\end{equation}
gezeigt werden ($f(n) \sim g(n) :\Leftrightarrow \lim_{n\rightarrow
  \infty} f(n)/g(n) = 1$).
\end{enumerate}
\end{korollar}
\begin{proof}
\begin{enumerate}
\item
Ein Binomialkoeffizient der Gestalt von (\ref{ersteUngl}) bzw.\
(\ref{zweiteUngl}) kann umgeschrieben werden ($l=n+d-1$, $k=m-1$) als
\begin{eqnarray*}
\bino{l+k}{k} = \frac{\prod_{j=1}^k (l+k)}{\prod_{j=1}^k k}
= \prod_{j=1}^k (1+\frac{l}{k}).
\end{eqnarray*}
Nach der Ungleichung vom arithmetischen und geometrischen Mittel gilt
\[
\sqrt[k]{\prod_{j=1}^k (1+\frac{l}{k})} < \frac{1}{k}\left[k + l \left(\sum_{j=1}^k
  \frac{1}{j} \right)\right],
\]
weiters
\begin{eqnarray*}
\sum_{j=1}^k \frac{1}{j} &<& 1 + \int_1^k \frac{\dx}{x} \\
&=& 1 + \ln k,
\end{eqnarray*}
weil Erstere eine Untersumme für das Integral ist.
Insgesamt gibt das
\[
\bino{l+k}{k} < \left[1+l \frac{1 + \ln k}{k}\right]^k
\]
bzw.
\[
\bino{n+d+m-2}{m-1} < \left[1+(n+d-1) \frac{1 + \ln (m-1)}{m-1}\right]^{m-1}.
\]
Der Rest folgt analog.
\item
Für hinreichend große $n$ ist der Fehlerterm (\ref{zweiteUngl}) für
$m=d$ dominant und mit
\[
\lim_{n\rightarrow \infty} \bino{n+2d-2}{d-1} \Big/ n^{d-1} = \frac{1}{(d-1)!}
\]
folgt die Behauptung, da es nur einen $d$-faktorigen Fehlerterm gibt.
\item
Ist keine Information über $s_l$ verfügbar, kann man (\ref{absEst})
nur mit dem Absolutbetrag der einzelnen Summanden abschätzen und
handelt sich den Faktor $5^d$ von Satz \ref{zweiteOrdnung} ein.
Wenn die $s_l$ hingegen eine gemeinsame Asymptotik haben, können die wechselnden
Vorzeichen in der binomischen Summe ausgenutzt werden.
In der Tat gilt unter der Stetigkeitsannahme für $\gamma_{1,\dots,m}$
\begin{equation}
\label{limit}
\lim_{n\rightarrow \infty} \frac{s_n}{\bino{n+m-1}{m-1}} =
\gamma_{1,\ldots,m}(0,\ldots,0) =: \gamma_0.
\end{equation}
Das gilt es zunächst zu zeigen (wenn keine Verwechslung möglich ist,
wird der Index von $\gamma_{1,\ldots,m}$ weggelassen, also ab jetzt
schlicht $\gamma$). Sei dazu $\epsilon>0$ beliebig und
\[
c := \sup_{0\le h_1,\ldots,h_m \le 1} |\gamma(h_1,\ldots,h_m)-\gamma_0|.
\]
Wegen
der Stetigkeit von $\gamma$ kann $n_0$ so gewählt werden, dass
\[
\forall i_k \ge n_0, 1\le k \le m: \quad
|\gamma(2^{-i_1},\ldots,2^{-i_m})-\gamma_0| \le \frac{\epsilon}{2}
\]
und danach $n$ so groß, dass
\[
N_0 := \bino{n-k n_0+m-1}{m-1} \ge \left(1-\frac{\epsilon}{c}\right)
\bino{n+m-1}{m-1} =: \left(1-\frac{\epsilon}{c}\right) N.
\]
Letzteres geht, weil
\[
\bino{n-k n_0+m-1}{m-1} \Big/ \bino{n+m-1}{m-1} = \prod_{j=1}^{m-1}
\left(1-\frac{k n_0}{n+j} \right) \rightarrow 1 \text{ für }
n\rightarrow \infty.
\]
Die Idee ist jetzt zu zeigen, dass der Beitrag der Summanden, die
nicht in  einer $\epsilon$-Umgebung von $\gamma_0$ liegen,
vernachlässigt werden kann. Das legt eine Aufspaltung in
\[
s_n = \sum_{\scriptsize \begin{array}{c}\sum_{k} i_k =n \\ \forall k: i_k \ge n_0
\end{array}}
\gamma(2^{-i_1},\ldots,2^{-i_m})
 \;\;\; +
\sum_{\scriptsize \begin{array}{c}\sum_{k} i_k =n \\ \exists k: i_k < n_0
\end{array}}
\gamma(2^{-i_1},\ldots,2^{-i_m})
\]
nahe.
Wegen
\[
\sum_{\scriptsize \begin{array}{c}\sum_{k} i_k =n \\ \forall k: i_k \ge n_0
\end{array}} 1
=
\sum_{\scriptsize \begin{array}{c}\sum_{k} i_k =n-m n_0 \\ \forall k: i_k \ge 0
\end{array}} 1
= N_0
\]
gilt schließlich
\begin{eqnarray*}
s_n - \gamma_0 N =
 \sum_{\scriptsize
  \begin{array}{c}\sum_{k} i_k =n \\ \forall k: i_k \ge n_0
\end{array}} \!\!\!\!\!\!
\left(\gamma(2^{-i_1},\ldots,2^{-i_m})-\gamma_0\right)
+ \!\!\!\!\!\!
\sum_{\scriptsize
  \begin{array}{c}\sum_{k} i_k =n \\ \exists k: i_k < n_0
\end{array}} \!\!\!\!\!\!
\left(\gamma(2^{-i_1},\ldots,2^{-i_m})-\gamma_0\right)
\end{eqnarray*}
und damit
\begin{eqnarray*}
\left|s_n - \gamma_0 N\right| &\le& 
  \frac{\epsilon}{2} N + c \left(N-N_0\right) \\
&\le& \frac{\epsilon}{2} N + c \frac{\epsilon}{2c} N \\
&=& \epsilon N.
\end{eqnarray*}
Division durch $N$ liefert die Behauptung (\ref{limit}).

Daher gilt asymptotisch
\[
\left(\Delta_n-3\right)^{m-1} s_{n+d-m}
\sim \gamma_0 N \sum_{i=0}^{m-1} \bino{m-1}{i} (-4)^{m-1-i} =
\gamma_0 \bino{n+m-1}{m-1} (-3)^{m-1}
\]
bzw.~exakter
\begin{equation}
\label{epsinequ}
\forall \epsilon>0 \;\, \exists N \;\, \forall n\ge N: \quad 
|\left(\Delta_n-3\right)^{m-1} s_{n+d-m}| \le \gamma_0 \bino{n+m-1}{m-1}
3^{m-1} (1+\epsilon).
\end{equation}
Letzteres gilt nicht für $\gamma_0 = 0$. In diesem
Fall, der ungünstig wechselnde Vorzeichen der $s_l$ nicht ausschließt,
gilt aber die stärkere Aussage
\[
\forall \epsilon>0 \;\, \exists N \;\, \forall n\ge N: \quad 
|\left(\Delta_n-3\right)^{m-1} s_{n+d-m}| \le \epsilon \bino{n+m-1}{m-1}
5^{m-1},
\]
die bzgl.~diesem Term auf höhere Konvergenzordnung führt und
hier nicht weiter betrachtet wird.

%Sei nun $N$ so gewählt, dass (\ref{epsinequ}) für
%alle $\bino{d}{m}$ $m$-stufigen Fehlerterme gilt, sodass man insgesamt
%erhält ($\gamma_0 \le K$)
%\begin{eqnarray*}
%|u-u_n| \le \frac{K}{4^d}  4^{-n} \sum_{m=1}^d 3^m \bino{n+m-1}{m-1}
%\bino{d}{m} (1+\epsilon).
%\end{eqnarray*}
In allen anderen Fällen ist asymptotisch der Fehlerterm für $m=d$ entscheidend, was die
Aussage liefert.
%&<& \frac{K}{4^d}  4^{-n} \bino{n+d-1}{d-1} \sum_{m=1}^d 3^m
%\bino{d}{m} (1+\epsilon) \\
%&=& \frac{K}{4^d}  4^{-n} \bino{n+d-1}{d-1} (4^d-1) (1+\epsilon) \\
%&<& \frac{K}{(d-1!)} 4^{-n} (n+d-1)^{d-1} \left(1-4^{-d} \right) (1+\epsilon).
%\end{eqnarray*}
%Da
%\[
%\frac{(n+d-1)^{d-1}}{n^{d-1}} \rightarrow 1 \text{ für } n\rightarrow \infty,
%\]
%kann man $\epsilon$ und $N$ von Anfang an so wählen, dass
%\[
%|u-u_n| \le K \frac{n^{d-1}}{(d-1)!} 4^{-n} \quad \forall n\ge N.
%\]
\end{enumerate}
\end{proof}

In Anbetracht von (\ref{asymptImpro}) und (\ref{traum}) stellt man
fest, dass die Vorfaktoren von $4^{-n}$
mit $d\rightarrow \infty$ gegen $0$ streben. Das ist aber wohlgemerkt
nur eine asymptotische Aussage, die unter anderem dadurch erreicht
wurde, dass $(n+d-1)/n \rightarrow 1$, also $n$ insbesondere im
Vergleich zu $d$ groß ist, sodass man in höheren Dimensionen immer später
in diesen asymptotischen Bereich kommt.

In dieser Verschiebung um $d-1$ versteckt sich auch die Tatsache, dass
die Kombinationslösung eine linear (mit $d$) ansteigende Zahl an
Gitterstufen enthält.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Diss/VeroeffentlichteVersion/diss"
%%% End: 


==> out <==
This is e-TeX, Version 3.14159-2.1 (Web2C 7.4.5)
entering extended mode
(./error.tex
LaTeX2e <2001/06/01>
Babel <v3.7h> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, catalan, croatian, czech, danish, dutch, finnish, greek, iceland
ic, irish, italian, latin, magyar, norsk, norsk, portuges, romanian, russian, s
lovak, slovene, spanish, swedish, turkish, ukrainian, nohyphenation, loaded.
\@input{Header.aux}
(./Header.tex (/usr/share/texmf/tex/latex/koma-script/scrartcl.cls
Document Class: scrartcl 2003/01/31 v2.9n LaTeX2e KOMA document class
(/usr/share/texmf/tex/latex/koma-script/scrlfile.sty
Package scrlfile, 2003/01/31 v2.9n LaTeX2e KOMA package
                  Copyright (C) Markus Kohm

) (/usr/share/texmf/tex/latex/base/size12.clo)
(/usr/share/texmf/tex/latex/koma-script/typearea.sty
Package typearea, 2003/01/31 v2.9n LaTeX2e KOMA package
                  Copyright (C) Frank Neukam, 1992-1994
                  Copyright (C) Markus Kohm, 1994-2002

)) (/usr/share/texmf/tex/latex/misc/a4wide.sty
(/usr/share/texmf/tex/latex/ntgclass/a4.sty))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/amscls/amsthm.sty)
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty)
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty)
(/usr/share/texmf/tex/latex/base/latexsym.sty)
(/usr/share/texmf/tex/latex/graphics/epsfig.sty
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/config/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def))))
(/usr/share/texmf/tex/latex/base/exscale.sty)
(/usr/share/texmf/tex/latex/misc/psfrag.sty)
(/usr/share/texmf/tex/latex/misc/isolatin1.sty
ISO-latin-1 input coding, version 0.9 of 1-Jun-1992.) (./fixme.sty)
(/usr/share/texmf/tex/latex/misc/placeins.sty)
(/usr/share/texmf/tex/latex/tools/afterpage.sty)
(/usr/share/texmf/tex/generic/thumbpdf/thumbpdf.sty

Package thumbpdf Warning: Thumbnail data file `error.tpm' not found.

) (/usr/share/texmf/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf/tex/latex/config/hyperref.cfg)
Implicit mode ON; LaTeX internals redefined
(/usr/share/texmf/tex/latex/misc/url.sty))
*hyperref using driver hdvips*
(/usr/share/texmf/tex/latex/hyperref/hdvips.def
(/usr/share/texmf/tex/latex/hyperref/pdfmark.def))
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf/tex/latex/base/ulasy.fd)

Package amsthm Warning: Unknown theoremstyle `bemerkung' on input line 135.

) (./error.aux) (/usr/share/texmf/tex/latex/hyperref/nameref.sty) (./error.out)
 (./error.out)

Package FiXme: `change font' on input line 12.


Package hyperref Warning: No destination for bookmark of \addcontentsline,
(hyperref)                destination is added on input line 12.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.

[1] (./tableau.tex) (./gridgrids.tex) [2] [3]

LaTeX Font Warning: Command \tiny invalid in math mode on input line 232.

[4] [5]

Package FiXme: `advection formulation' on input line 361.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.


LaTeX Warning: Marginpar on page 6 moved.


Package FiXme: `space-time' on input line 363.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.

[6] [7]

LaTeX Font Warning: Command \tiny invalid in math mode on input line 521.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 582.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 595.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 616.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 622.

[8]

LaTeX Font Warning: Command \tiny invalid in math mode on input line 646.


Overfull \hbox (45.42267pt too wide) in alignment at lines 682--689
 [][][] []
[9] [10]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 939.



LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 959.



LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 968.


[11]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1055
.


Package FiXme: `attention when changing intro' on input line 1103.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.

[12]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1192
.

[13]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1267
.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 1296.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1318
.

[14]

LaTeX Font Warning: Command \tiny invalid in math mode on input line 1339.


Overfull \hbox (16.80211pt too wide) in alignment at lines 1333--1344
 [][][] []

Overfull \hbox (2.61975pt too wide) in alignment at lines 1346--1351
 [][][] []

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1359
.


Overfull \hbox (3.52576pt too wide) detected at line 1364
\OML/cmm/m/it/12 ^^K[]\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 x\OT1/cmr/m/n/12 ; \OML
/cmm/m/it/12 h[]; [] ; h[]\OT1/cmr/m/n/12 ) = [] [] []   [] [] [][]  [][] \OML/
cmm/m/it/12 w[]\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 x\OT1/cmr/m/n/12 ; \OT1/cmr/bx
/n/12 h\OT1/cmr/m/n/12 )

Package FiXme: `details?' on input line 1384.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.

[15]

Package FiXme: `details of K?' on input line 1424.


Package hyperref Warning: bookmark level for unknown fixme defaults to 0.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 1434.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1467
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1500
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1504
.

[16]

LaTeX Font Warning: Command \tiny invalid in math mode on input line 1525.


LaTeX Font Warning: Command \tiny invalid in math mode on input line 1572.

[17]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1623
.

[18]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1755
.

[19]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1795
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 1843
.

[20] [21] [22] [23] [24] <convPlotsDim.eps> <convElsPlotsDim.eps>
<convSFPlotsDim.eps> <convElsSFPlotsDim.eps> [25]
Overfull \hbox (22.85278pt too wide) in paragraph at lines 2224--2235
 [][] 
[26] [27] (./error.bbl [28])

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2444
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2454
.

[29] [30] [31]

LaTeX Font Warning: Command \small invalid in math mode on input line 2606.


LaTeX Font Warning: Command \small invalid in math mode on input line 2607.


LaTeX Font Warning: Command \small invalid in math mode on input line 2617.


LaTeX Font Warning: Command \small invalid in math mode on input line 2618.

[32] [33]

LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2732
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2736
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2742
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2745
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2766
.


LaTeX Font Warning: Command \scriptsize invalid in math mode on input line 2770
.

[34]

Package FiXme Summary: Number of notes: 0,
(FiXme)                Number of warnings: 0,
(FiXme)                Number of errors: 0,
(FiXme)                Number of fatal errors: 6,
(FiXme)                Total: 6.

[35] (./error.aux) )
(see the transcript file for additional information)
Output written on error.dvi (35 pages, 204980 bytes).
Transcript written on error.log.

